Optimal Sampling and Scheduling for Timely Status Updates in Multi-source Networks

We consider a joint sampling and scheduling problem for optimizing data freshness in multi-source systems. Data freshness is measured by a non-decreasing penalty function of \emph{age of information}, where all sources have the same age-penalty function. Sources take turns to generate update packets, and forward them to their destinations one-by-one through a shared channel with random delay. There is a scheduler, that chooses the update order of the sources, and a sampler, that determines when a source should generate a new packet in its turn. We aim to find the optimal scheduler-sampler pairs that minimize the total-average age-penalty at delivery times (Ta-APD) and the total-average age-penalty (Ta-AP). We prove that the Maximum Age First (MAF) scheduler and the zero-wait sampler are jointly optimal for minimizing the Ta-APD. Meanwhile, the MAF scheduler and a relative value iteration with reduced complexity (RVI-RC) sampler are jointly optimal for minimizing the Ta-AP. The RVI-RC sampler is based on a relative value iteration algorithm whose complexity is reduced by exploiting a threshold property in the optimal sampler. Finally, a low-complexity threshold-type sampler is devised via an approximate analysis of Bellman's equation. This threshold-type sampler reduces to a simple water-filling sampler for a linear age-penalty function.

==> sections/Discussion.tex <==
\section{Discussion}\label{Disc}
In this section, we discuss our results and compare it with prior works. 
\subsection{Preemption vs. Non-Preemption}
In the conclusion of \cite[Appendix]{CostaCodreanuEphremides_TIT}, the authors claimed that "In  the  LCFS  system  with  preemption  we  expect  that,  for  very large  arrival  rates,  the  age  would  increase  without  bound,  as  no  packet  finishes  service''. This claim is correct when the packet service times are NBU. As we will see in Fig. \ref{avg_peak_age3}, the age of the preemptive LCFS policy grows to infinity at high traffic intensity for gamma distributed service times. However, preemption does not increase the age for exponential service times, because the remaining service times of a preempted packet has the same distribution with the service time of a new packet. In Theorem \ref{thm1}, we have proven that the preemptive LCFS policy is age-optimal for exponential service times and general system parameters. In Theorem 3(a) of \cite{RYatesTIT16}, Yates and Kaul showed that the average age of the preemptive LCFS policy is a decreasing function of the traffic intensity $\rho$ in M/M/1 queues as $\rho$ grows to infinite. 

%On one hand, this contradicts our results in Theorem \ref{thm1}, in which we showed that the LCFS system with preemption can, indeed, achieve age-optimality for all arrival rates among all causal policies when the service times are exponentially distributed and the update packets arrive in the order of their generation times. Moreover, the study in \cite{RYatesTIT16} showed that the preemptive LCFS policy achieves bounded average age for all arrival rates when the service times are exponentially distributed. However, for non-exponential service time, the age of the preemptive LCFS policy could blow up at high traffic intensity (as we will see in Fig. \ref{avg_peak_age3}). This is because the packet service times are no longer memoryless. Thus, high traffic intensity leads to increased preemption rate which, in turn, leads to no packet completes service. Hence, the inter-departure times increase causing the rise in the age. From this, we can deduce that the age performance of the prmp-LGFS-R policy depends essentially on the service time distribution.

In addition, the study in \cite{Gamma_dist} characterized the age for LCFS systems with and without preemption for  gamma distributed service times. In \cite[Numerical Results]{Gamma_dist}, the authors showed that the non-preemptive LCFS policy can achieve better average age performance than the preemptive LCFS policy. In this paper, we further show that the non-prmp-LGFS-R policy is within a small constant gap from the optimum expected average age for all NBU service time distributions, which include gamma distribution as one example.

%In addition, the study in \cite{Gamma_dist} characterized the age for LCFS systems with and without preemption when the service time is gamma distributed (gamma distribution belongs to the class of NBU distributions). In \cite[Numerical Results]{Gamma_dist}, the authors showed that the non-preemptive policy can achieve better average age than the preemptive one. In this paper, we showed that the non-prmp-LGFS-R policy can come close to age-optimal when the service time is NBU distributed. More specifically, the non-prmp-LGFS-R is within a small age gap from the optimum expected average age for NBU service times.

\subsection{Replication vs. Non-Replication}
The replication technique has gained significant attention in recent years to reduce the delay in queueing systems \cite{Chen_queue_coding,yin_data_retrieve,sun2016delay}. However, under some system settings, replications may worsen the delay performance. In particular, it was shown in \cite{sun2016delay} that replication policies are far from the optimum delay for NBU service time distributions. A simple explanation of this result is as follows: Let $X_1, X_2, \ldots, X_m$ be i.i.d. NBU random variables with mean $\mathbb{E}[X_l]=\mathbb{E}[X]<\infty$. From the properties of the NBU distributions, we can obtain \cite{joshi2017efficient}
\begin{equation}\label{NBUproperty_delay}
\mathbb{E}[\min_{l=1,\ldots,m}X_l]\geq \frac{\mathbb{E}[X]}{m}.
\end{equation}
Now, if $X_l$ represents the packet service time of server $l$, then the left-hand side of \eqref{NBUproperty_delay} represents the mean service time (the mean time spent by each server per packet) when each packet is replicated to all servers; and the right-hand side of \eqref{NBUproperty_delay} represents the mean service time when there is no replication. This gives insight why packet replication can worsen the delay performance when the service time is NBU. Somewhat to our surprise, we found in this paper that the non-prmp-LGFS-R policy is near-optimal in minimizing the age, even for NBU service time distributions. The intuition behind this result is that the age is affected by the freshness of the delivered packets irrelevant to the total number of delivered packets. In other words, to reduce the age, we need to deliver the freshest packet as soon as possible. Also, it is obvious that 
\begin{equation}
\mathbb{E}[\min_{l=1,\ldots,m}X_l]\leq\mathbb{E}[X].
\end{equation}
Thus, packet replication can help in this direction by exploiting the diversity provided by multiple servers. 
\subsection{New-Worse-than-Used service time distributions}
Another important class of distributions that are more general than exponential is New-Worse-than-Used (NWU) distributions. The definition of the NWU distributions is as follows: 
\begin{definition}  \textbf{New-Worse-than-Used distributions:} Consider a non-negative random variable $Z$ with CCDF $\bar{F}(z)=\mathbb{P}[Z>z]$. Then, $Z$ is \textbf{New-Worse-than-Used (NWU)} if for all $t,\tau\geq0$
\begin{equation}\label{NWU_Inequality}
\bar{F}(\tau +t)\geq \bar{F}(\tau)\bar{F}(t).
\end{equation} 
\end{definition}
Examples of NWU distributions include hyperexponential distribution, Weibull distribution with $c <1$, etc. A  random variable is both NBU and NWU if, and only if, it is exponential. We investigated whether age-optimality can be achieved when the service times are NWU. We figured out that no policy can achieve optimality when the service times are NWU. To clarify this claim, let us consider the following example.

 \begin{figure*}[!tbp]
 \centering
 \subfigure[Case 1: Preemption is allowed.]{
  \includegraphics[scale=0.3]{figure/NWU.eps}
   \label{1a}
   }
 \subfigure[Case 2: Preemption is not allowed.]{
  \includegraphics[scale=0.3]{figure/NWU2.eps}
   \label{2b}
   }
   \caption{Illustration of policies $\pi$ and $\pi'$ in the Example }
   \label{fig:samp_path_NBU}
\end{figure*}
\textbf{Example:}
\emph{Consider a single server queue with $U(0)=0$ for all policies. We first consider the case where preemption is allowed. Suppose that the policies $\pi$ and $\pi'$ start to process packet 1 at time 0, as shown in  Fig. \ref{1a}. Suppose that at time $\delta$, packet 2 with $s_2<s_1$ arrives at the system. Since $s_1>s_2$, an intuitive action is to keep processing the fresh packet (packet 1) and ignore the old packet (packet 2). We will show that this decision may not achieve lower age. Suppose that policy $\pi'$ preempts the processing of packet 1 and starts to serve packet 2 at time $\delta$ and completes the service of packet 2 at time $\gamma$, as shown in  Fig. \ref{1a}. Let $R_1$ represent the remaining service time to complete packet 1 at time $\delta$ under policy $\pi$. Suppose that the server has spent $\chi$ ($\chi\geq 0$) seconds on processing packet 1 by time $\delta$ in policy $\pi$. Define $X_1=\chi+R_1$ as the service time of packet 1 under policy $\pi$ and $X_2=\gamma-\delta$ as the service time of packet 2 under policy $\pi'$. Then, the CCDF of $R_1$ is given by
\begin{equation}\label{ex_NWU_1}
\mathbb{P}[R_1>t]=\mathbb{P}[(X_1-\chi)>t\vert X_1>\chi].
\end{equation}
Because the packet service times are NWU, we can obtain that for all $t, \chi\geq 0$
\begin{equation}\label{ex_NWU_2}
\mathbb{P}[(X_1-\chi)>t\vert X_1>\chi]=\mathbb{P}[(X_2-\chi_1)>t\vert X_2>\chi_1]\geq\mathbb{P}[X_2>t].
\end{equation}
Combining \eqref{ex_NWU_1} and \eqref{ex_NWU_2}, we get
\begin{equation}\label{ex_NWU_3}
R_1\geq_{\text{st}}X_2.
\end{equation}
This means that the completion time of packet 2 under policy $\pi'$ is stochastically smaller than the completion time of packet 1 under policy $\pi$, as shown in  Fig. \ref{1a}. Thus, policy $\pi'$ can obtain lower age at time $\gamma$ than policy $\pi$, i.e., we have
\begin{equation}
\Delta_\pi(\gamma)=\gamma\geq\gamma-s_2=\Delta_{\pi'}(\gamma).
\end{equation}}

\emph{Now, we proceed to the case where preemption is not allowed. We will show that a non-work-conserving policy can obtain lower age than the work-conserving one. Suppose that policy $\pi$ starts processing packet 1 at time 0; and policy $\pi'$ does idle the server until time $\delta$, then assigns packet 2 to the server, as shown in Fig. \ref{2b}. We assume here that $0=a_1<a_2\leq\delta$ and $s_2>s_1$. By the same argument as in the first case, we can show that the completion time of packet 2 under policy $\pi'$ is stochastically smaller than the completion time of packet 1 under policy $\pi$, as shown in Fig. \ref{2b}. This means that the non-work-conserving policy $\pi'$ can obtain a lower age than policy $\pi$.}

This example shows that age-optimality is extremely hard to be achieved within the policy space that includes all causal policies when the service times are NWU distributed. However, we showed in \cite{multihop_optimal} that optimality can be achieved for general service time in single server queues among all non-preemptive work-conserving policies.

==> sections/Thro-Delay-analysis.tex <==
\section{Throughput-Delay Analysis}\label{thro-anal}
In this section, we investigate the throughput and delay performances of the proposed policies. We first consider the exponential service time distribution. Then, we generalize the service time distribution to the NBU distributions. We need the following definitions:
\begin{definition}\textbf{Throughput-optimality:} A policy is said to be \textbf{throughput-optimal}, if it maximizes the expected number of delivered packets among all causal policies. 
\end{definition}
The average delay under policy $\pi$ is defined as
\begin{equation}\label{average_delay}
D_{\text{avg}}(\pi)=\frac{1}{n}\sum_{i=1}^n[c_i(\pi)-a_i],
\end{equation}
where the delay of packet $i$ under policy $\pi$ is $c_i(\pi)-a_i$.\footnote{The $\limsup$ operator is enforced on the right hand side of \eqref{average_delay} if $n\rightarrow\infty$.}
\begin{definition}\textbf{Delay-optimality:} A policy is said to be \textbf{delay-optimal}, if it minimizes the expected average delay among all causal policies. 
\end{definition}
\subsection{Exponential Service Time Distribution}
We study the throughput and delay performance of the prmp-LGFS-R policy when the service times are exponentially distributed and \emph{i.i.d.} across time and servers. 
The delay and throughput performances of the prmp-LGFS-R policy are characterized as follows:
\begin{theorem}\label{thm2th}
Suppose that the packet service times are exponentially distributed and \emph{i.i.d.} across time and servers, then for all $\mathcal{I}$ such that $B=\infty$, the prmp-LGFS-R policy is throughput-optimal and delay-optimal among all policies in $\Pi_m$.
\end{theorem}

\begin{proof}
In particular, any work-conserving policy is throughput-optimal and delay-optimal. The proof details are provided in Appendix~\ref{Appendix_C}.
\end{proof}

% \textbf{Remark.} Because the packet service times are \emph{i.i.d.} across time and servers and the CDF $\bar{F}$ is continuous, the probability for any two servers to complete their packets at the same time is zero. Therefor, similar to the proof of Theorem \ref{thm2th}, we can prove that the prmp-LGFS-R policy is throughput-optimal and mean-delay-optimal among all policies in $\Pi$.

\subsection{NBU Service Time Distributions}
Now, we consider class of NBU service time distributions. We study the throughput and delay performance of the non-prmp-LGFS-R policy when the maximum replication degree is 1 (i.e., there is no replication). Moreover, we assume that all packets have identical size.
%We need the following definition:
%\begin{definition}\textbf{Near delay-optimal:} A policy is said to be \emph{near delay-optimal}, if it is within a constant additive delay gap from the optimum for minimizing the mean average delay (For more details, see \cite{sunnear}).
%\end{definition}
The delay and throughput performances of the non-prmp-LGFS-R policy are characterized as follows:
\begin{theorem}\label{thmNBU1th}
Suppose that the packet service times are NBU and \emph{i.i.d.} across time and servers, then for all $\mathcal{I}$ such that $B=\infty$ and $r=1$, the non-prmp-LGFS-R policy is throughput-optimal and delay-optimal among all non-preemptive policies in $\Pi_{1}$.
\end{theorem}

Indeed, when the packet service times are NBU and preemption is not allowed, any non-preemptive work-conserving policy in $\Pi_{1}$ is throughput and delay optimal. The proof is omitted because it is similar to that of Theorem \ref{thm2th}. The only difference is that using the property of NBU distributions, we can show that service idling in any non-work-conserving policy leads to delayed packet departure instants, which in turn worsens its throughput and delay performance. 

%We omit the proof of throughput-optimality of the non-prmp-LGFS-R policy, because it is similar to that of Theorem \ref{thm2th}. 
% The near delay-optimality of  non-prmp-LGFS-R policy is proven in \cite{sunnear}.



